Subtraction of temperature induced phase noise in the LISA frequency band

Temperature fluctuations are expected to be one of the limiting factors for gravitational wave detectors in the very low frequency range. Here we report the characterisation of this noise source in the LISA Pathfinder optical bench and propose a method to remove its contribution from the data. Our results show that temperature fluctuations are indeed limiting our measurement below one millihertz, and that their subtraction leads to a factor 5.6 (15 dB) reduction in the noise level at the lower end of the LISA measurement band 10^{-4} Hz, which increases to 20.2 (26 dB) at even lower frequencies, i.e., 1.5x10^{-5} Hz. The method presented here can be applied to the subtraction of other noise sources in gravitational wave detectors in the general situation where multiple sensors are used to characterise the noise source.

==> include/._analysis.tex.1.4 <==
We tested the method in the LISA Pathfinder optical bench~\cite{Heinzel03,Heinzel05},
the closest optical system to the final LISA Pathfinder satellite~\cite{Armano09}.
In our setup, test masses are substituted by fixed mirrors so only the interferometric
metrology subsystem is tested; none of the required drag-free technology
used in the final mission is part of the experiment. Although the test-bed has
shown the required performance in the LISA Pathfinder frequency band,
$\rm 1\,mHz \le f \le 1\,Hz$~\cite{Heinzel05}, our main aim was to determine
to what extent our measurements were limited by environmental temperature fluctuations and,
also, to evaluate this noise contribution in the LISA band. In order to do so,
we measured the temperature in four different locations of our setup, 
as shown in Fig.~\ref{fig.scheme}.
%one sensor was attached to each mounting structure supporting the mirrors, a third
%sensor was attached to the side slab flange ---a metallic structure 
%from which the optical bench will be supported inside the satellite thermal shield---  
%and a fourth which measures the temperature in the laboratory.
We initially tested the method using a long data set ($2~\times10^5$\,s),  where the
interferometer was running without active noise suppression control loops.
With the temperature coupling characterised and the method verified, we then
proceeded to subtract the temperature contribution in a shorter, low noise data
segment to characterise the impact of this contribution when the interferometer
is performing according to the mission requirements, reaching 1 $\rm pm/\sqrt{Hz}$
at 0.1\,Hz.
\begin{figure}[t]
\includegraphics[width=\textwidth]{figs/OBsetup_temperature_fig1.png}
\caption{Schematic representation (not to scale) of the location of the temperature
sensors in the LISA Pathfinder optical bench. One sensor was attached 
to each mounting structure supporting the mirrors, a third
sensor was attached to the side slab flange ---a metallic structure 
from which the optical bench will be supported inside the satellite thermal shield---  
and a fourth (not shown) measured the temperature in the laboratory.
\label{fig.scheme}}
\end{figure}
%

Before analysing, data needed to be resampled onto a common time grid.  Both the
interferometer data (with a sampling frequency of $\rm f_s = 32.47 \, Hz$), and
the temperature data (with $\rm f_s = 1.3 \, Hz$)  were down-sampled to $\rm f_s
= 1\,Hz$.  The temperature sensor data were interpolated to the new time grid with
the new sampling frequency, from 1.3 to 1 \,Hz. In the interferometer case,
the data are first down-sampled by a factor of 10 in order to ease data handling,
and then resampled to the common grid.
To determine the interdependence between temperature
measured at different locations we use the coherence function, which contains
the information of the correlation between two data sets $X$ and $Y$ as,
\begin{equation}
\gamma^2_{XY}(f) = \frac{|S_{XY}(f)|^2}{S_{XX}(f) S_{YY}(f)},
\end{equation}
where $S_{XX}(f)$ and $S_{XY}(f)$ refer to the power spectrum and cross-power spectrum
respectively. In this first step of our analysis, we compute the coherence
between each pair of temperature sensors, $\gamma^2_{T_i T_j}(f)|_{i \ne j}$.  
\begin{figure}[t]
\begin{center}
\caption{Temperature to interferometer transfer functions for the four sensors 
in the setup. Errors and fitted model are only shown for the transfer function 
that shows the highest contribution, 
the one coming from the sensor in the first mirror (M1). 
  \label{fig.tf}}
\includegraphics[width=0.8\textwidth]{figs/2008-09-12_17-19_tf_magnitude_fig2a}
\\[0.1cm]
\includegraphics[width=0.8\textwidth]{figs/2008-09-12_17-19_tf_phase_fig2b}
\end{center}
\end{figure}
Results show that the four temperatures are strongly correlated ($\gamma^2_{T_{i} T_j}(f)
\simeq 1$), in the low frequency  frequency band ($f < \rm 1\,mHz$), and
the correlation drops off rapidly above these frequencies. The analysis shows that,
at the low frequencies of interest, the four measurements contain mostly the same information.
While at higher frequencies environmental temperature fluctuations can
be screened by the vacuum tank; in the low frequency region these fluctuations
pass directly through the setup (although delayed, as we show below).

\begin{figure*}[t]
\includegraphics[width=0.8\textwidth]{figs/phase_time_subtracted_fig3a}
\includegraphics[width=0.8\textwidth]{figs/phase_frequency_subtracted_fig3b}
\caption{Temperature noise subtraction for a two days measurement without
control loops suppressing the interferometric noise contributions. 
{\it Left:} Time domain data series for the two most rellevant temperature sensors 
and the interferometer read out. We also show interferometer data after 
subtracting the information contained in the two previous temperatures sensors.
{\it Right:} Frequency domain analysis. For comparison, we show the
requirement on interferometric noise in the LISA Pathfinder mission.}
\label{fig.subs}
\end{figure*}
Even though the four measurements contain similar temperature contribution at low
frequencies, they do not contribute with the same strength to the interferometric
measurement. To show that, we use the transfer function between the temperature
data and interferometer data,
\begin{equation}
 H_{\varphi T_{i}}(f) = \frac{S_{\varphi T_i}(f)}{S_{\varphi \varphi}(f)}, \quad i=1,2,3,4
\end{equation}
In Fig.~\ref{fig.tf} we show these transfer functions for each sensor; the sensor
attached to the first test mass (M1) shows a higher contribution
with respect to the other
%namely a low pass filter profile with roughly a 4\,rad/K
%gain at low frequencies and a pole at around 0.1\,mHz 
---numerical values for
the transfer function are shown in Tab. \ref{tbl.tf}. 
Also, from a linear fit to the phase of this transfer function in the low frequency
band we obtain the group delay of the filter. For our setup, the interferometer
to temperature fluctuations below the millihertz frequency band is delayed by $1430
\pm 70$\,s with respect to the actual time of temperature measurement. To bound
the uncertainty of our transfer function estimates, we compute the error on the transfer
function as~\cite{Bendat}
%\begin{subeqnarray}
%\sigma\left[ |\hat H_{\varphi T}| \right] & \simeq &  \frac{\left[ 1- \hat \gamma^2_{ \varphi T}(f) \right]^{1/2}}{[ |\hat \gamma_{\varphi T}(f)| \, \sqrt{2\,n_d}}  \label{eq.errmag}  \\
%\sigma\left[ \hat \theta ( H_{\varphi T}) \right] &\simeq & \sin^{-1} \left( \sigma\left[ |\hat H_{\varphi T}| \right]  \right) 
%\end{subeqnarray}
\begin{equation}
\sigma\left[ | H_{\varphi T_i}| \right]  \simeq  \sigma\left[ \theta ( H_{\varphi T_i}) \right]  \simeq
 \frac{\left[ 1- \gamma^2_{ \varphi T_i}(f) \right]^{1/2}}{[ | \gamma_{\varphi T_i}(f)| \, \sqrt{2\,n_d}}  \label{eq.errmag}  
\end{equation}
where $n_d$ is the number of averages used to compute the transfer function estimates.
The error on the transfer function already
contains the information about the correlation between the temperature and
the interferometer in the form of the coherence function $\gamma^2_{ \varphi T_i}(f)$.
By doing this, we ensure that our error estimate takes into account the
correlation between temperature and interferometric phase fluctuations. We note
that, in our analysis, and as shown in Tab. \ref{tbl.tf}, this correlation is valid
for $\rm f \le 0.5\,mHz$. Therefore, the frequency region
where we would expect a noise reduction after subtraction of this contribution would
be below the LISA Pathfinder measuring band, but directly affecting a LISA-like measurement.
\begin{table}[b]
\caption{Numerical values for the transfer function correspondin to the sensor in the
first mirror mount (M1) and associated errors. 
Last column shows the coherence function. \label{tbl.tf}}
\begin{center}
\begin{tabular}{ccc}
Frequency [Hz] &  $|\hat H_{\varphi T}|$ [rad/K]  & $\hat \gamma_{\varphi T}(f)$  \\
\hline
 $1.6 \times 10^5$    & $4.5 \pm 0.5$   & 0.97 \\
 % $5.1 \times 10^5$    & $5.1  \pm 0.6$  & 0.96 \\
 $1.1 \times 10^4$    & $4.5 \pm 0.6$   & 0.91  \\
 $2.6 \times 10^4$    & $2.7 \pm 0.5$   & 0.85\\
 $5.3 \times 10^4$    & $1.6 \pm 2.8$   & 0.12 \\
 $1.0 \times 10^3$    &  $1.4 \pm 2.6$  & 0.10  \\
 $2.5 \times 10^3$    & $0.5 \pm 6.5$ & 0.01\\
\end{tabular}
\end{center}
\end{table} 
%      1.55005115168801e-05           4.4872139214792          0.52265546676561          0.97392306654291
%      5.07989440469883e-05          5.09312313751554         0.613004290718616          0.95918328371233
%      0.000109026877586206          4.51607547683581         0.634280358525189         0.913914718538724
%      0.000258741654058045          2.74562628299583         0.459725969252425         0.847426206740851
%      0.000526890352139399          1.61567999327024          2.81911346145805         0.121286756946792
%      0.00103635016387276          1.46074565220661          2.63403303676713         0.100734448928743
%       0.00246343032263182         0.503323359851059          6.45431111091562        0.0114971333985326
%      0.00499264285390534         0.469132598061002          3.59762401626114        0.016297919327881 
%

Before removing the contribution from the temperature sensors, we proceed to estimate
the expected noise reduction. To do this, we compute the conditioned
spectra~\cite{Bendat}
%\begin{equation}
% S_{\varphi \varphi \cdot T}(f)  =   S_{\varphi \varphi}(f) \, \left[ 1 - \gamma^2_{ \varphi T}(f) \right],
%\label{eq.cond}
\begin{equation}
 S_{\varphi \varphi \cdot T_{i}!}(f)  =   S_{\varphi \varphi \cdot T_{(i-1)}!}(f) \, \left( 1 - \gamma^2_{ \varphi T_i \cdot T_{(i-1)}! }(f) \right),
\label{eq.cond}
\end{equation} 
which corresponds to the phase noise spectrum, $S_{\varphi \varphi}(f)$, when contributions
from temperature sensors are recursively removed, by linear subtraction. Accordingly, 
the coherence appearing in the equation is the partial coherence 
$\gamma^2_{ \varphi T_i \cdot T_{(i-1)}!}$,
i.e. the coherence between $\varphi$ and $T_i$, 
once all contribution from previous $i-1$ sensors, $T_{(i-1)!}$, are subtracted.
Results are shown in Fig.
\ref{fig.subs} (right panel) where the curve labelled as `prediction' shows the
conditioned spectrum in equation (\ref{eq.cond}) 
for the two sensors with stronger contributions 
(we also performed the analysis for a third but the coherence with 
the interferometer was already too small to show any improvement).
As expected, a coherent subtraction
of the temperature contribution would reduce the noise level at frequencies
$\rm f \leq 0.4\,mHz$.  According to this first analysis, the subtraction
of the contribution contained in these two sensors
would reduce the instrument noise floor by a factor 5.6 (15\,dB) at the very low end
of the LISA measurement band, $\rm f = 0.1\,mHz$. The factor increases up to 20.2
(26\,dB) at the lowest frequency bin, $\rm f = 15\,\mu Hz$.

Subtraction must be done necessarily in time domain.  For this reason we have previously
resampled both data streams  with the same sampling frequency and on a synchronous
time grid. 
%The procedure we follow, however, differs from the linear subtraction
%scheme assumed to compute the predicted value in the frequency domain.
As previously shown, the relation between temperature and phase read out is better
described by their frequency domain description.  We then translate this transfer
function into a digital filter, i.e., a recursive relation that allows us
to include a certain dynamical response and, in particular, a delayed action of
the temperature upon the interferometer. The tool used here is the vector fitting
algorithm~\cite{Gustavsen99}  
%---details of the implementation can be found in~\cite{Ferraioli10}---
which allows us to fit the measured transfer function in terms
of N poles, $p_k$, and residues , $z_k$, 
\begin{equation}  
h_{\varphi T_i}(z^{-1}) = \sum_{k=1}^{N} \frac{r_k }{1-p_k\,z^{-1}}   
\label{eq.respol} 
\end{equation}

Since our previous analysis showed that the temperature contribution to the interferometer
is relevant in a frequency range up to $\rm \simeq1\,mHz$, we fit the
transfer function up to this frequency. Figure \ref{fig.tf}  shows the fit result
with a 3rd order model. Once the digital filter is obtained, we filter the temperature
measurement with $h_{\varphi T_i}(z^{-1})$ to obtain the temperature contribution
to the interferometer, which we can then readily subtract from the original
measurement.
This procedure is performed initially considering the temperature reading
of the sensor attached to the mounting of the first mirror ($\rm T_{\rm M1}$). Then, the information
contained in the flange sensor ($\rm T_{\rm FL}$) is removed from the residual of the first subtraction.
\begin{figure}[t]
\includegraphics[width=\textwidth]{figs/tempsubtract_performance_fig4}
\caption{Temperature noise substraction for a data segment where
control loops were active, showing compliance with the Pathfinder interferometric 
noise requirement. }
\label{fig.subs_performance}
\end{figure}
%This procedure is shown in Fig.~\ref{fig.subs} where the time-domain
%representation clearly shows the effect of the subtraction in the long control-free 
%measurement. In the right panel, we compute the amplitude spectral density
%of the time-series using a log-frequency-based algorithm~\cite{Troebs06}.
As shown in Fig.~\ref{fig.subs}, the subtracted curve is in agreement with the 
one previously obtained in the frequency
domain analysis. We show, for comparison, the LISA Pathfinder interferometric
noise goal on the same plot. Since the control loops were not suppressing the
interferometric noise contributions, the measurement is above the goal. To further
investigate the temperature noise contribution in our setup we used the method
above to subtract the temperature noise contribution in a measurement where the
instrument was operating in closed-loop (all noise suppression on). The transfer
function is the same as the one previously evaluated since the setup remains
unchanged. As shown in Fig.~\ref{fig.subs_performance}, the effect of the subtraction
reduces the noise level at lower frequencies, $\rm f \leq 0.2\,mHz$, when compared 
with the control-free case although
the effect is stronger at $\rm f = 0.1\,mHz$, reducing the noise floor a factor
10 (20\,dB) after the subtraction. We notice as well that, according to
our current analysis, we can not attribute the corner in the low end of the LISA
Pathfinder measuring band, $\rm f \simeq 1\,mHz$, to temperature noise.  
% The subtracted
% curve and the associated error are consistent with the measured curve at
% those frequencies.

The analysis reported here characterises, for the first time, the low frequency temperature
coupling to an interferometric measurement in a realistic gravitational
wave instrumental setup. We also introduce a methodology to
clean the main measurement of this noise contribution by removing the
information contained in multiple sensors monitoring the experiment.
Once applied, the results confirm
the prediction obtained by a frequency domain noise projection. Results on the
LISA Pathfinder optical bench show that, when considering the temperature readings
in our current setup, the instrument performance is not affected in the Pathfinder measurement band
after the temperature noise subtraction, although it gives
a significant noise reduction at lower frequencies, and therefore this noise source has a direct
impact for LISA experiments. This is of relevance for any ground-based gravitational
 wave experiments aiming at low frequencies, and in particular for those testing
technologies for space-based gravitational wave observatories. The method
described above allows these experiments to compute a performance curve without
the limitation of the unavoidable temperature drifts, and it is as well extendable
to any frequency dependent contribution that is independently measurable
in gravitational wave experiments.


%
%\begin{table}[b]
%\caption{Numerical values for the measured phase noise spectrum, 
%$S^{1/2}_m$, compared with the spectrum after temperature substraction, $S^{1/2}_{T T}$. \label{tbl.nums2}}
%\begin{tabular}{cccc}
% Frequency [mHz] &  $S^{1/2}_{nT}$ [$\rm rad/\sqrt{Hz}$]  & $S^{1/2}_{nT}$ [$\rm rad/\sqrt{Hz}$]  \\
% \hline
% \hline
% 0.1 & 1.4 & $0.3 \pm 0.2$ &\\
% 0.2 & $5 \times 10^{-2}$ & $(8 \pm 10) \times 10^{-3}$ & \\
%0.6 & $3 \times 10^{-3}$ & $(2 \pm 1) \times 10^{-3}$ \\
%1 & $1.9 \times 10^{-3}$ & $(1.7 \pm 0.1) \times 10^{-3}$ & \\
% \end{tabular}
% \end{table}


==> include/analysis_conditioned.tex <==


\section{Temperature noise subtraction}
%
\begin{figure*}[t]
\begin{center}
\includegraphics[width=0.55\textwidth]{figs/phase_time_subtracted_fig3a}
\includegraphics[width=0.42\textwidth]{figs/phase_frequency_subtracted_fig3b}
\caption{Temperature noise subtraction for a two days measurement without
control loops suppressing the interferometric noise contributions. 
{\it Left:} Time domain data series for the two most rellevant temperature sensors 
and the interferometer read out. We also show interferometer data after 
subtracting the information contained in the two previous temperatures sensors.
{\it Right:} Frequency domain analysis. For comparison, we show the
requirement on interferometric noise in the LISA Pathfinder mission.}
\label{fig.subs}
\end{center}
\end{figure*}
\subsection{Frequency domain analysis}
Before removing the contribution from the temperature sensors, we proceed to estimate
the expected noise reduction. To do this, we compute the conditioned
spectra~\cite{Bendat}
%%\begin{equation}
%% S_{\varphi \varphi \cdot T}(f)  =   S_{\varphi \varphi}(f) \, \left[ 1 - \gamma^2_{ \varphi T}(f) \right],
%%\label{eq.cond}
%\begin{equation}
% S_{\varphi \varphi \cdot T_{i}!}(f)  =   S_{\varphi \varphi \cdot T_{(i-1)}!}(f) \, \left( 1 - \gamma^2_{ \varphi T_i \cdot T_{(i-1)}! }(f) \right),
%\label{eq.cond}
%\end{equation} 
%which corresponds to the phase noise spectrum, $S_{\varphi \varphi}(f)$, when contributions
%from temperature sensors are recursively removed, by linear subtraction. Accordingly, 
%the coherence appearing in the equation is the partial coherence 
%$\gamma^2_{ \varphi T_i \cdot T_{(i-1)}!}$,
%i.e. the coherence between $\varphi$ and $T_i$, 
%once all contribution from previous $i-1$ sensors, $T_{(i-1)!}$, are subtracted.
Results are shown in Fig.
\ref{fig.subs} (right panel) where the curve labelled as `prediction' shows the
conditioned spectrum in equation (\ref{eq.cond}) 
for the two sensors with stronger contributions 
(we also performed the analysis for a third but the coherence with 
the interferometer was already too small to show any improvement).
As expected, a coherent subtraction
of the temperature contribution would reduce the noise level at frequencies
$\rm f \leq 0.4\,mHz$.  According to this first analysis, the subtraction
of the contribution contained in these two sensors
would reduce the instrument noise floor by a factor 5.6 (15\,dB) at the very low end
of the LISA measurement band, $\rm f = 0.1\,mHz$. The factor increases up to 20.2
(26\,dB) at the lowest frequency bin, $\rm f = 15\,\mu Hz$.

\subsection{Time domain analysis}
Subtraction must be done necessarily in time domain.  For this reason we have previously
resampled both data streams  with the same sampling frequency and on a synchronous
time grid. 
%The procedure we follow, however, differs from the linear subtraction
%scheme assumed to compute the predicted value in the frequency domain.
As previously shown, the relation between temperature and phase read out is better
described by their frequency domain description.  We then translate this transfer
function into a digital filter, i.e., a recursive relation that allows us
to include a certain dynamical response and, in particular, a delayed action of
the temperature upon the interferometer. The tool used here is the vector fitting
algorithm~\cite{Gustavsen99}  
%---details of the implementation can be found in~\cite{Ferraioli10}---
which allows us to fit the measured transfer function in terms
of N poles, $p_k$, and residues , $z_k$, 
\begin{equation}  
h_{\varphi T_i}(z^{-1}) = \sum_{k=1}^{N} \frac{r_k }{1-p_k\,z^{-1}}   
\label{eq.respol} 
\end{equation}

Since our previous analysis showed that the temperature contribution to the interferometer
is relevant in a frequency range up to $\rm \simeq1\,mHz$, we fit the
transfer function up to this frequency. Figure \ref{fig.tf}  shows the fit result
with a 3rd order model. Once the digital filter is obtained, we filter the temperature
measurement with $h_{\varphi T_i}(z^{-1})$ to obtain the temperature contribution
to the interferometer, which we can then readily subtract from the original
measurement.
This procedure is performed initially considering the temperature reading
of the sensor attached to the mounting of the first mirror ($\rm T_{\rm M1}$). Then, the information
contained in the flange sensor ($\rm T_{\rm FL}$) is removed from the residual of the first subtraction.
\begin{figure}[t]
\includegraphics[width=0.49\textwidth]{figs/tempsubtract_performance_fig4}
\caption{Temperature noise substraction for a data segment where
control loops were active, showing compliance with the Pathfinder interferometric 
noise requirement. }
\label{fig.subs_performance}
\end{figure}
%This procedure is shown in Fig.~\ref{fig.subs} where the time-domain
%representation clearly shows the effect of the subtraction in the long control-free 
%measurement. In the right panel, we compute the amplitude spectral density
%of the time-series using a log-frequency-based algorithm~\cite{Troebs06}.
As shown in Fig.~\ref{fig.subs}, the subtracted curve is in agreement with the 
one previously obtained in the frequency
domain analysis. We show, for comparison, the LISA Pathfinder interferometric
noise goal on the same plot. Since the control loops were not suppressing the
interferometric noise contributions, the measurement is above the goal. To further
investigate the temperature noise contribution in our setup we used the method
above to subtract the temperature noise contribution in a measurement where the
instrument was operating in closed-loop (all noise suppression on). The transfer
function is the same as the one previously evaluated since the setup remains
unchanged. As shown in Fig.~\ref{fig.subs_performance}, the effect of the subtraction
reduces the noise level at lower frequencies, $\rm f \leq 0.2\,mHz$, when compared 
with the control-free case although
the effect is stronger at $\rm f = 0.1\,mHz$, reducing the noise floor a factor
10 (20\,dB) after the subtraction. We notice as well that, according to
our current analysis, we can not attribute the corner in the low end of the LISA
Pathfinder measuring band, $\rm f \simeq 1\,mHz$, to temperature noise.  
% The subtracted
% curve and the associated error are consistent with the measured curve at
% those frequencies.


%
%\begin{table}[b]
%\caption{Numerical values for the measured phase noise spectrum, 
%$S^{1/2}_m$, compared with the spectrum after temperature substraction, $S^{1/2}_{T T}$. \label{tbl.nums2}}
%\begin{tabular}{cccc}
% Frequency [mHz] &  $S^{1/2}_{nT}$ [$\rm rad/\sqrt{Hz}$]  & $S^{1/2}_{nT}$ [$\rm rad/\sqrt{Hz}$]  \\
% \hline
% \hline
% 0.1 & 1.4 & $0.3 \pm 0.2$ &\\
% 0.2 & $5 \times 10^{-2}$ & $(8 \pm 10) \times 10^{-3}$ & \\
%0.6 & $3 \times 10^{-3}$ & $(2 \pm 1) \times 10^{-3}$ \\
%1 & $1.9 \times 10^{-3}$ & $(1.7 \pm 0.1) \times 10^{-3}$ & \\
% \end{tabular}
% \end{table}


==> include/analysis_old.tex <==
We tested the method in the LISA Pathfinder optical bench~\cite{Heinzel03,Heinzel05},
the closest optical system to the final LISA Pathfinder satellite~\cite{Armano09}.
In our setup, test masses are substituted by fixed mirrors so only the interferometric
metrology subsystem is tested; none of the required drag-free technology
used in the final mission is part of the experiment. Although the test-bed has
shown the required performance in the LISA Pathfinder frequency band,
$\rm 1\,mHz \le f \le 1\,Hz$~\cite{Heinzel05}, our main aim was to determine
to what extent our measurements were limited by environmental temperature fluctuations and,
also, to evaluate this noise contribution in the LISA band. In order to do so,
we measured the temperature in four different locations of our setup, 
as shown in Fig.~\ref{fig.scheme}.
%one sensor was attached to each mounting structure supporting the mirrors, a third
%sensor was attached to the side slab flange ---a metallic structure 
%from which the optical bench will be supported inside the satellite thermal shield---  
%and a fourth which measures the temperature in the laboratory.
We initially tested the method using a long data set ($2~\times10^5$\,s),  where the
interferometer was running without active noise suppression control loops.
With the temperature coupling characterised and the method verified, we then
proceeded to subtract the temperature contribution in a shorter, low noise data
segment to characterise the impact of this contribution when the interferometer
is performing according to the mission requirements, reaching 1 $\rm pm/\sqrt{Hz}$
at 0.1\,Hz.
\begin{figure}[t]
\includegraphics[width=0.49\textwidth]{figs/OBsetup_temperature_fig1.png}
\caption{Schematic representation (not to scale) of the location of the temperature
sensors in the LISA Pathfinder optical bench. One sensor was attached 
to each mounting structure supporting the mirrors, a third
sensor was attached to the side slab flange ---a metallic structure 
from which the optical bench will be supported inside the satellite thermal shield---  
and a fourth (not shown) measured the temperature in the laboratory.
\label{fig.scheme}}
\end{figure}
%

Before analysing, data needed to be resampled onto a common time grid.  Both the
interferometer data (with a sampling frequency of $\rm f_s = 32.47 \, Hz$), and
the temperature data (with $\rm f_s = 1.3 \, Hz$)  were down-sampled to $\rm f_s
= 1\,Hz$.  The temperature sensor data were interpolated to the new time grid with
the new sampling frequency, from 1.3 to 1 \,Hz. In the interferometer case,
the data are first down-sampled by a factor of 10 in order to ease data handling,
and then resampled to the common grid.
To determine the interdependence between temperature
measured at different locations we use the coherence function, which contains
the information of the correlation between two data sets $X$ and $Y$ as,
\begin{equation}
\gamma^2_{XY}(f) = \frac{|S_{XY}(f)|^2}{S_{XX}(f) S_{YY}(f)},
\end{equation}
where $S_{XX}(f)$ and $S_{XY}(f)$ refer to the power spectrum and cross-power spectrum
respectively. In this first step of our analysis, we compute the coherence
between each pair of temperature sensors, $\gamma^2_{T_i T_j}(f)|_{i \ne j}$.  
\begin{figure}[b]
\caption{Temperature to interferometer transfer functions for the four sensors 
in the setup. Errors and fitted model are only shown for the transfer function 
that shows the highest contribution, 
the one coming from the sensor in the first mirror (M1). 
  \label{fig.tf}}
\includegraphics[width=0.45\textwidth]{figs/2008-09-12_17-19_tf_magnitude_fig2a}
\\[0.1cm]
\includegraphics[width=0.45\textwidth]{figs/2008-09-12_17-19_tf_phase_fig2b}
\end{figure}
Results show that the four temperatures are strongly correlated ($\gamma^2_{T_{i} T_j}(f)
\simeq 1$), in the low frequency  frequency band ($f < \rm 1\,mHz$), and
the correlation drops off rapidly above these frequencies. The analysis shows that,
at the low frequencies of interest, the four measurements contain mostly the same information.
While at higher frequencies environmental temperature fluctuations can
be screened by the vacuum tank; in the low frequency region these fluctuations
pass directly through the setup (although delayed, as we show below).

\begin{figure*}[t]
\includegraphics[width=0.57\textwidth]{figs/phase_time_subtracted_fig3a}
\includegraphics[width=0.42\textwidth]{figs/phase_frequency_subtracted_fig3b}
\caption{Temperature noise subtraction for a two days measurement without
control loops suppressing the interferometric noise contributions. 
{\it Left:} Time domain data series for the two most rellevant temperature sensors 
and the interferometer read out. We also show interferometer data after 
subtracting the information contained in the two previous temperatures sensors.
{\it Right:} Frequency domain analysis. For comparison, we show the
requirement on interferometric noise in the LISA Pathfinder mission.}
\label{fig.subs}
\end{figure*}
Even though the four measurements contain similar temperature contribution at low
frequencies, they do not contribute with the same strength to the interferometric
measurement. To show that, we use the transfer function between the temperature
data and interferometer data,
\begin{equation}
 H_{\varphi T_{i}}(f) = \frac{S_{\varphi T_i}(f)}{S_{\varphi \varphi}(f)}, \quad i=1,2,3,4
\end{equation}
In Fig.~\ref{fig.tf} we show these transfer functions for each sensor; the sensor
attached to the first test mass (M1) shows a higher contribution
with respect to the other
%namely a low pass filter profile with roughly a 4\,rad/K
%gain at low frequencies and a pole at around 0.1\,mHz 
---numerical values for
the transfer function are shown in Tab. \ref{tbl.tf}. 
Also, from a linear fit to the phase of this transfer function in the low frequency
band we obtain the group delay of the filter. For our setup, the interferometer
to temperature fluctuations below the millihertz frequency band is delayed by $1430
\pm 70$\,s with respect to the actual time of temperature measurement. To bound
the uncertainty of our transfer function estimates, we compute the error on the transfer
function as~\cite{Bendat}
%\begin{subeqnarray}
%\sigma\left[ |\hat H_{\varphi T}| \right] & \simeq &  \frac{\left[ 1- \hat \gamma^2_{ \varphi T}(f) \right]^{1/2}}{[ |\hat \gamma_{\varphi T}(f)| \, \sqrt{2\,n_d}}  \label{eq.errmag}  \\
%\sigma\left[ \hat \theta ( H_{\varphi T}) \right] &\simeq & \sin^{-1} \left( \sigma\left[ |\hat H_{\varphi T}| \right]  \right) 
%\end{subeqnarray}
\begin{equation}
\sigma\left[ | H_{\varphi T_i}| \right]  \simeq  \sigma\left[ \theta ( H_{\varphi T_i}) \right]  \simeq
 \frac{\left[ 1- \gamma^2_{ \varphi T_i}(f) \right]^{1/2}}{[ | \gamma_{\varphi T_i}(f)| \, \sqrt{2\,n_d}}  \label{eq.errmag}  
\end{equation}
where $n_d$ is the number of averages used to compute the transfer function estimates.
The error on the transfer function already
contains the information about the correlation between the temperature and
the interferometer in the form of the coherence function $\gamma^2_{ \varphi T_i}(f)$.
By doing this, we ensure that our error estimate takes into account the
correlation between temperature and interferometric phase fluctuations. We note
that, in our analysis, and as shown in Tab. \ref{tbl.tf}, this correlation is valid
for $\rm f \le 0.5\,mHz$. Therefore, the frequency region
where we would expect a noise reduction after subtraction of this contribution would
be below the LISA Pathfinder measuring band, but directly affecting a LISA-like measurement.
\begin{table}[b]
\caption{Numerical values for the transfer function correspondin to the sensor in the
first mirror mount (M1) and associated errors. 
Last column shows the coherence function. \label{tbl.tf}}
\begin{center}
\begin{ruledtabular}
\begin{tabular}{ccc}
Frequency [Hz] &  $|\hat H_{\varphi T}|$ [rad/K]  & $\hat \gamma_{\varphi T}(f)$  \\
\hline
 $1.6 \times 10^5$    & $4.5 \pm 0.5$   & 0.97 \\
 % $5.1 \times 10^5$    & $5.1  \pm 0.6$  & 0.96 \\
 $1.1 \times 10^4$    & $4.5 \pm 0.6$   & 0.91  \\
 $2.6 \times 10^4$    & $2.7 \pm 0.5$   & 0.85\\
 $5.3 \times 10^4$    & $1.6 \pm 2.8$   & 0.12 \\
 $1.0 \times 10^3$    &  $1.4 \pm 2.6$  & 0.10  \\
 $2.5 \times 10^3$    & $0.5 \pm 6.5$ & 0.01\\
\end{tabular}
\end{ruledtabular}
\end{center}
\end{table} 
%      1.55005115168801e-05           4.4872139214792          0.52265546676561          0.97392306654291
%      5.07989440469883e-05          5.09312313751554         0.613004290718616          0.95918328371233
%      0.000109026877586206          4.51607547683581         0.634280358525189         0.913914718538724
%      0.000258741654058045          2.74562628299583         0.459725969252425         0.847426206740851
%      0.000526890352139399          1.61567999327024          2.81911346145805         0.121286756946792
%      0.00103635016387276          1.46074565220661          2.63403303676713         0.100734448928743
%       0.00246343032263182         0.503323359851059          6.45431111091562        0.0114971333985326
%      0.00499264285390534         0.469132598061002          3.59762401626114        0.016297919327881 
%

Before removing the contribution from the temperature sensors, we proceed to estimate
the expected noise reduction. To do this, we compute the conditioned
spectra~\cite{Bendat}
%\begin{equation}
% S_{\varphi \varphi \cdot T}(f)  =   S_{\varphi \varphi}(f) \, \left[ 1 - \gamma^2_{ \varphi T}(f) \right],
%\label{eq.cond}
\begin{equation}
 S_{\varphi \varphi \cdot T_{i}!}(f)  =   S_{\varphi \varphi \cdot T_{(i-1)}!}(f) \, \left( 1 - \gamma^2_{ \varphi T_i \cdot T_{(i-1)}! }(f) \right),
\label{eq.cond}
\end{equation} 
which corresponds to the phase noise spectrum, $S_{\varphi \varphi}(f)$, when contributions
from temperature sensors are recursively removed, by linear subtraction. Accordingly, 
the coherence appearing in the equation is the partial coherence 
$\gamma^2_{ \varphi T_i \cdot T_{(i-1)}!}$,
i.e. the coherence between $\varphi$ and $T_i$, 
once all contribution from previous $i-1$ sensors, $T_{(i-1)!}$, are subtracted.
Results are shown in Fig.
\ref{fig.subs} (right panel) where the curve labelled as `prediction' shows the
conditioned spectrum in equation (\ref{eq.cond}) 
for the two sensors with stronger contributions 
(we also performed the analysis for a third but the coherence with 
the interferometer was already too small to show any improvement).
As expected, a coherent subtraction
of the temperature contribution would reduce the noise level at frequencies
$\rm f \leq 0.4\,mHz$.  According to this first analysis, the subtraction
of the contribution contained in these two sensors
would reduce the instrument noise floor by a factor 5.6 (15\,dB) at the very low end
of the LISA measurement band, $\rm f = 0.1\,mHz$. The factor increases up to 20.2
(26\,dB) at the lowest frequency bin, $\rm f = 15\,\mu Hz$.

Subtraction must be done necessarily in time domain.  For this reason we have previously
resampled both data streams  with the same sampling frequency and on a synchronous
time grid. 
%The procedure we follow, however, differs from the linear subtraction
%scheme assumed to compute the predicted value in the frequency domain.
As previously shown, the relation between temperature and phase read out is better
described by their frequency domain description.  We then translate this transfer
function into a digital filter, i.e., a recursive relation that allows us
to include a certain dynamical response and, in particular, a delayed action of
the temperature upon the interferometer. The tool used here is the vector fitting
algorithm~\cite{Gustavsen99}  
%---details of the implementation can be found in~\cite{Ferraioli10}---
which allows us to fit the measured transfer function in terms
of N poles, $p_k$, and residues , $z_k$, 
\begin{equation}  
h_{\varphi T_i}(z^{-1}) = \sum_{k=1}^{N} \frac{r_k }{1-p_k\,z^{-1}}   
\label{eq.respol} 
\end{equation}

Since our previous analysis showed that the temperature contribution to the interferometer
is relevant in a frequency range up to $\rm \simeq1\,mHz$, we fit the
transfer function up to this frequency. Figure \ref{fig.tf}  shows the fit result
with a 3rd order model. Once the digital filter is obtained, we filter the temperature
measurement with $h_{\varphi T_i}(z^{-1})$ to obtain the temperature contribution
to the interferometer, which we can then readily subtract from the original
measurement.
This procedure is performed initially considering the temperature reading
of the sensor attached to the mounting of the first mirror ($\rm T_{\rm M1}$). Then, the information
contained in the flange sensor ($\rm T_{\rm FL}$) is removed from the residual of the first subtraction.

%This procedure is shown in Fig.~\ref{fig.subs} where the time-domain
%representation clearly shows the effect of the subtraction in the long control-free 
%measurement. In the right panel, we compute the amplitude spectral density
%of the time-series using a log-frequency-based algorithm~\cite{Troebs06}.
As shown in Fig.~\ref{fig.subs}, the subtracted curve is in agreement with the 
one previously obtained in the frequency
domain analysis. We show, for comparison, the LISA Pathfinder interferometric
noise goal on the same plot. Since the control loops were not suppressing the
interferometric noise contributions, the measurement is above the goal. To further
investigate the temperature noise contribution in our setup we used the method
above to subtract the temperature noise contribution in a measurement where the
instrument was operating in closed-loop (all noise suppression on). The transfer
function is the same as the one previously evaluated since the setup remains
unchanged. As shown in Fig.~\ref{fig.subs_performance}, the effect of the subtraction
reduces the noise level at lower frequencies, $\rm f \leq 0.2\,mHz$, when compared 
with the control-free case although
the effect is stronger at $\rm f = 0.1\,mHz$, reducing the noise floor a factor
10 (20\,dB) after the subtraction. We notice as well that, according to
our current analysis, we can not attribute the corner in the low end of the LISA
Pathfinder measuring band, $\rm f \simeq 1\,mHz$, to temperature noise.  
% The subtracted
% curve and the associated error are consistent with the measured curve at
% those frequencies.

The analysis reported here characterises, for the first time, the low frequency temperature
coupling to an interferometric measurement in a realistic gravitational
wave instrumental setup. We also introduce a methodology to
clean the main measurement of this noise contribution by removing the
information contained in multiple sensors monitoring the experiment.
Once applied, the results confirm
the prediction obtained by a frequency domain noise projection. Results on the
LISA Pathfinder optical bench show that, when considering the temperature readings
in our current setup, the instrument performance is not affected in the Pathfinder measurement band
after the temperature noise subtraction, although it gives
a significant noise reduction at lower frequencies, and therefore this noise source has a direct
impact for LISA experiments. This is of relevance for any ground-based gravitational
 wave experiments aiming at low frequencies, and in particular for those testing
technologies for space-based gravitational wave observatories. The method
described above allows these experiments to compute a performance curve without
the limitation of the unavoidable temperature drifts, and it is as well extendable
to any frequency dependent contribution that is independently measurable
in gravitational wave experiments.

\begin{figure}[t]
\includegraphics[width=0.45\textwidth]{figs/tempsubtract_performance_fig4}
\caption{Temperature noise substraction for a data segment where
control loops were active, showing compliance with the Pathfinder interferometric 
noise requirement. }
\label{fig.subs_performance}
\end{figure}

%
%\begin{table}[b]
%\caption{Numerical values for the measured phase noise spectrum, 
%$S^{1/2}_m$, compared with the spectrum after temperature substraction, $S^{1/2}_{T T}$. \label{tbl.nums2}}
%\begin{tabular}{cccc}
% Frequency [mHz] &  $S^{1/2}_{nT}$ [$\rm rad/\sqrt{Hz}$]  & $S^{1/2}_{nT}$ [$\rm rad/\sqrt{Hz}$]  \\
% \hline
% \hline
% 0.1 & 1.4 & $0.3 \pm 0.2$ &\\
% 0.2 & $5 \times 10^{-2}$ & $(8 \pm 10) \times 10^{-3}$ & \\
%0.6 & $3 \times 10^{-3}$ & $(2 \pm 1) \times 10^{-3}$ \\
%1 & $1.9 \times 10^{-3}$ & $(1.7 \pm 0.1) \times 10^{-3}$ & \\
% \end{tabular}
% \end{table}


==> include/analysis_optimal.tex <==
\section{Spectral analysis}

Once we have characterised our system, our next step is to disentangle the temperature contribution from the interferometer measurement. We will proceed in two different ways: first, solving the linear system and obtaining a set of optimal transfer function and second, applying a conditioned scheme, which proceeds by solving the linear system for each individual contribution. We describe both in the following. 

\subsection{Optimal spectral analysis}

In order to obtain the system of linear equations that will describe our problem we start
with Eq.~\ref{eq.system},
\begin{equation}
\Phi(\omega) = \sum^q_{i=1} H_i(\omega)\,T_i(\omega) + N(\omega)
\end{equation}  
where, if we multiply $\Phi(\omega)$ by its complex conjugate $\Phi(\omega)^*$, 
and taking expected values we obtain 
\begin{equation}
S_{nn} = S_{\Phi\Phi} - \sum_{i=1}^q H_i\,S_{\Phi T_i} - \sum_{i=1}^q H^*_j\,S_{T_j \Phi} + \sum_{i=j}^q\sum_{i=1}^q H^*_j\,H_i\,S_{T_j T_i}
\end{equation}
The optimal solution for this system of equations which minimise $S_{NN}$ 
over all possible choices of $H_i$ is found by setting 
\begin{equation}
\frac{\partial S_{nn}}{\partial H_j} = 0 , \quad \frac{\partial S_{nn}}{\partial H^*_j} = 0
\end{equation}
which leads to~\cite{Bendat}
\begin{equation}
S_{T_j \Phi} = \sum_{i=1}^q H_i\,S_{T_j T_i} , \quad j = 1, 2, \ldots q
\end{equation}
which can be solved for $H_i$, since $S_{\Phi T_i}$  and $S_{T_i T_j}$ are known. In our particular case  this turns into a system of 4 equations,
%\begin{eqnarray}
%S_{T_1 \Phi} =  H_1\, S_{T_1 T_1}  + H_2\, S_{T_1 T_2} + H_3\, S_{T_1 T_3}+ H_4 \, S_{T_1 T_4} \nonumber \\
%S_{T_2\Phi} =   H_1\, S_{T_2 T_1}  + H_2\, S_{T_2 T_2} + H_3\, S_{T_2 T_3}+ H_4 \, S_{T_2 T_4} \nonumber\\
%S_{T_3 \Phi} =  H_1\, S_{T_3 T_1}  + H_2\, S_{T_3 T_2} + H_3\, S_{T_3 T_3}+ H_4 \, S_{T_3 T_4} \nonumber\\
%S_{T_4 \Phi} =  H_1\, S_{T_4 T_1}  + H_2\, S_{T_4 T_2} + H_3\, S_{T_4 T_3}+ H_4 \, S_{T_4 T_4} \nonumber\\
%\end{eqnarray}
which leads to analytical solutions for $H_i,\; i = 1,2,3,4$. The expressions for $H_i$, which we do not reproduce here, require to compute 24 terms for each transfer function, each term containing a product of 4 spectral densities. In the following section we introduce a sequential method which allows to handle simpler equations, leading to equivalent results.

\subsection{Conditioned spectral analysis}

A second possible approach is to subtract (in a linear least square sense) 
one by one those contributions perturbing our measurement. This scheme 
leads to simpler expressions, which will 
allow the derivation of the digital filters required to clean the data in time domain.
This approach, know as \emph{conditioned} spectral analysis, derives 
the dependence between one of the input and the output when the other 
inputs are turned off, implicitly requiring here that the correlations between 
inputs are turned off as well. 
To implement this scheme we compute the conditioned
spectra~\cite{Bendat}
\begin{equation}
 S_{\Phi \Phi \cdot T_{i}!}  =   S_{\Phi \Phi \cdot T_{(i-1)}!} \, \left( 1 - \gamma^2_{ \Phi T_i \cdot T_{(i-1)}! } \right),
\label{eq.cond}
\end{equation} 
where $i=1,2,\ldots q$. This quantity corresponds to the phase noise spectrum, $S_{\Phi \Phi}(f)$, when contributions from temperature sensors, $T_{i}$ are recursively removed by linear least squares.
Appendix \ref{sec:condExpr} shows the expressions for the q =4 case. 
Accordingly to the current scheme, the coherence appearing in the equation is the partial coherence,
\begin{equation}
\gamma^2_{ \varphi T_i \cdot T_{(i-1)}!} = \frac{|S_{T_i \Phi \cdot T_{(i-1)}!}|^2}{S_{T_i T_i \cdot T_{(i-1)}} S_{\Phi \Phi \cdot T_{(i-1)}}}
\end{equation}

i.e. the coherence between $\varphi$ and $T_i$, 
once all contribution from previous $i-1$ sensors, $T_{(i-1)!}$, are subtracted.


==> include/macros.tex <==
\newcommand{\martin}[1]{\textcolor{blue}{\textit{Martin: #1}}}
\newcommand{\miquel}[1]{\textcolor{red}{\textit{Miquel: #1}}}
\newcommand{\christian}[1]{\textcolor{green}{\textit{Ch.: #1}}}

\newcommand{\etc}{\textit{etc}}
\newcommand{\ie}{\textit{i.e.}}
\newcommand{\da}{\textsc{LTPDA}}
\newcommand{\code}[1]{\texttt{#1}}
\newcommand{\tbd}[0]{\textcolor{red}{TBD}}
\newcommand{\ltpda}[0]{\textsc{LTPDA}}

\newcommand{\note}[1]{\textcolor{blue}{(#1)}}



